SWEET: Serving the Web by Exploiting Email Tunnels

Open communication over the Internet poses a serious threat to countries with repressive regimes, leading them to develop and deploy censorship mechanisms within their networks. Unfortunately, existing censorship circumvention systems do not provide high availability guarantees to their users, as censors can identify, hence disrupt, the traffic belonging to these systems using today's advanced censorship technologies. In this paper we propose SWEET, a highly available censorship-resistant infrastructure. SWEET works by encapsulating a censored user's traffic to a proxy server inside email messages that are carried over by public email service providers, like Gmail and Yahoo Mail. As the operation of SWEET is not bound to specific email providers we argue that a censor will need to block all email communications in order to disrupt SWEET, which is infeasible as email constitutes an important part of today's Internet. Through experiments with a prototype of our system we find that SWEET's performance is sufficient for web traffic. In particular, regular websites are downloaded within couple of seconds.

==> files/conclusions.tex <==

\section{Conclusions}\label{sec:conclusions}



In this paper, we presented \name, a deployable system for unobservable communication with Internet destinations.
\name works by tunneling network traffic through widely-used public email
services such as Gmail, Yahoo Mail, and Hotmail.
Unlike recently-proposed schemes that require a collection of ISPs to instrument router-level
modifications in support of covert communications, our approach can be deployed
through a small applet running at the user's end host, and a remote email-based proxy,
simplifying deployment.
Through an implementation and evaluation in a wide-area deployment, we find that while \name incurs some additional latency in communications, these overheads are low enough to be used for interactive accesses to web services. We feel our work may serve to accelerate deployment of censorship-resistant services in the wide area, guaranteeing high availability.
% matt: if results don't come in on time, you may want to cut this last bit

%Our design tunnels traffic through widely-used public email services, obviating
%the need to rely on hard-to-deploy changes to the Internet's physical infrastructure


==> files/discussions.tex <==


\section{Discussions and comparisons}\label{sec:discussions}
% security analysis
In this section we evaluate \name's circumvention capabilities  by discussing important features that are essential for an effective circumvention.

%In Section~\ref{sec:goals}, we listed the main features in evaluating a censorship circumvention system. In the following, we discuss these features for the \name system designed in this paper.

\subsection{Unobservability and the use of encryption}\label{sec:enc}

We say a circumvention tool provides unobservability if censors are not able to identify the users of that tool by monitoring the Internet traffic of their citizens. Unobservability has been considered in designing several recent circumvention systems~\cite{Karlin2011, Wustrow2011,Houmansadr2011a} as a mechanism to ensure the availability of the service.

Usage unobservability can be a very desirable property to users
living under repressive regimes, as it can reduce a user's risk of
suspicion by the government. However, if desired, \name users may
disable unobservability while retaining availability. This provides
the benefit of reduced latency. It comes at the expense of
observability, but users in some environments may wish to retain
reliable anonymous communications yet do not fear reprisal from their
government.
%We believe that usage unobservability is only demanded by special citizens, like political activists, but not ordinary citizens. A recent study~\cite{circumvention-servey}  conducted  on the use of circumvention tools in several countries shows that, in choosing a circumvention tool, users give the most preference to the ease of use and availability of the tool, rather than its security. In fact, none of the top listed tools in the study provide usage unobservability \cite{circumvention-servey}.
%As a second argument to support this point, there are no media reports about ordinary citizens being arrested/punished solely for using anti-censorship technologies. 
\name users have the option to use \name in a highly unobservable manner, or to trade off unobservability for better communication performance.
%Based on this, we make usage unobservability as an optional attribute to \name users.
More specifically, the use of an encryption-enabled email service (e.g., Gmail, Hushmail\footnote{\url{www.hushmail.com}}) with \name provides usage unobservability for the user, as the censor will not be able to see the recipient's email address, e.g., {\tt tunnel@sweet.org}.  On the other side, the use of plaintext email services (e.g., Yahoo!, Hotmail) provides better availability as repressive regimes occasionally disrupt or block the access to encryption-enabled  services, including encrypted emails  (yet they do not block all email communications). As a recent instance, Iran blocked all HTTPS connections of its citizen during the second week of February 2012 \cite{Iran-block-https}, the anniversary of  Iran's green movement in 2009.
In addition, while using an encryption-enabled email, to ensure unobservability the user's email traffic patterns should mimic that of normal email communications, e.g., to defeat traffic analysis by a censor; this limits the bandwidth available to the user, as discussed in Section~\ref{sec:trafanal}.


%\subsubsection{Traffic Analysis}


\subsection{Availability}\label{sec:availability}
\name's availability is tied to the assumption discussed previously that a censor is not willing to block \emph{all} email communications, as it would degrade the usability of the Internet for its users. As the use of \name does not require an email account with any specific email provider, users can always find an email service to get connected to \name.

IP filtering and DNS hijacking techniques would not be able to stop \name traffic as a \name user's traffic is destined to her public email provider, but not to an IP address or nameserver belonging to \name system.
Another technique used by today's sophisticated censors is deep packet inspection (DPI).
The use of encryption-enabled email renders DPI ineffective, as the email headers get encrypted and the DPI will not be able to analyze the email headers in order to detect the email addresses of \name, to hence block the traffic.
In the case of plaintext emails, to defeat DPI \name server can provide different \emph{email aliases} to different users or to change its public email address frequently. Note that generating email aliases has no cost for \name server and can be done with no limit. In the worst case, a user can obtain her specialized email address through an out of band channel, or by connecting through a encryption-enabled email account (as mentioned before the DPI is ineffective on encryption-enabled emails).


\begin{comment}
\name's unobservability, as discussed above,
prevents a censor from using common censorship techniques to block a client's
access to \name: first, there is no overt connection to known IP addresses of
\name that can be blocked by a censor, and second, the use of encrypted emails
renders deep packet-inspection (DPI) techniques ineffective.
A censor also is not able to block \name using her knowledge about the publicly known  design
of the \name system. More specifically, since
the design of \name is not bound to any specific email provider, in order to
block \name based on the \name's design knowledge a censor needs to block all email communication, which
significantly degrades the usability of the Internet and is very unlikely to be
adopted  by a censoring ISP.
\end{comment}

As another approach  for disrupting the operation of \name, a censor
might try to launch a denial-of-service (DoS) attack  on \name server.
The common techniques for DoS attacks, e.g., ICMP flooding and SYN flooding, can be mitigated by protecting the \name server using up-to-date firewalls.
Alternatively, a malicious entity (e.g., a censor) can try to exhaust  the \name service
by sending disruptive traffic through the email communication channel of \name. In other words,
a censor can play the role of a \name client and send Internet traffic through its \name client software in a way
that breaks or overloads  the \name server. As an example, the attacker can flood the \name's SOCKS proxy
by initiating many incomplete SOCKS connections, or sending SYN floods.
A censor could send such attacking requests  on behalf of a number of rogue (non-existing) email addresses, to render an email blacklist maintained   by \name server ineffective in preventing such attacks.
As a result, \name server should deploy effective mechanisms to protect against possible
DoS attacks. One effective mechanism is to require  a new user to register her email address
with \name server prior to her first use of \name. Such registration can be  performed in an unobservable manner
by \name's client software through the email communication channel (see Section~\ref{sec:server}).
Also, to ensure the quality of service for all users, the \name server can limit the use of \name
by putting a cap on the volume of traffic communicated by each registered email address.



\subsection{Other properties of \name}
%\begin{itemize}

\paragraphb{Confidentiality:}
As mentioned before, \name encrypts the tunneled traffic, i.e., the email attachments are encrypted using a key shared between a user and \name server. This ensures the confidentiality of \name user communications from any entity wiretapping the traffic, including the censorship authorities and the public email provider. Note that the email attachments are encrypted even if the user to choose a plaintext email service. To make a connection confidential from \name server the user can use an end-to-end encryption with the final destination, e.g., by using HTTPS. Alternatively, a user can use \name to connect to another circumvention system, like Anonymizer~\cite{circumvention-servey}, to ensure confidentiality from \name server.


%\paragraph{Unobservability:} A \name client's covert communication is encapsulated inside
%benign-looking encrypted emails. In other words, a user's \name traffic does not generate
%traffic patterns that can be observed by censoring ISPs. More specifically, a \name user does
%not make connections to specific end-host or proxy IP addresses. Also, the email communications  %of
%a \name user is not bound to a particular email provider, and the user can use an email account
%with \textit{any} email provider, and any type of email communication
%(i.e., through  either webmail or email protocols).






\paragraphb{\bf Ease of deployment:}
We argue that \name can be easily deployed on the Internet and provide
service to a wide range of users.
First of all, \name is low-cost and needs few resources for deployment. It can be deployed using
a single server that runs a few light-weight processes, including a mail server and a SOCKS proxy. To service in a large scale \name server can be deployed in
a distributed manner by several machines in different geographic locations.
Secondly, the operation of \name is standalone and does not rely on collaboration from other entities, e.g., end-hosts or ISPs.
This provides a significant advantage to recent research that relies on
collaboration from ISPs \cite{Wustrow2011,Karlin2011,Houmansadr2011a}, or end-hosts~\cite{collage,infranet}.
%The need for such a collaboration is a challenge regarding several recent circumvention systems \cite{Wustrow2011,Karlin2011,Houmansadr2011a}, due to the lack of strong incentives for the third-parties, which  questions their near-future real-world deployment.
In fact, the easy setup and low-resources of \name's deployment allows it to be implemented by individuals with different levels of technical expertise. For instance, an ordinary home user can deploy a personal \name server to help her friends in censored regions evade censorship, or a corporate network can setup such system for its agents residing in a censored country.



\paragraphb{\bf User convenience:}
As mentioned before, a recent study \cite{circumvention-servey} surveying the use of circumvention tools in censored countries shows that users give the most preference to the ease of use when choosing a  circumvention tool.  The use of \name is simple and requires few resources from  a client.
A \name client only needs to
install the provided client software, that can be obtained from out-of-band channels like social networks or downloaded from the Internet. Due to its simple design, an expert user can also develop the client software herself.
In addition to \name software, the user needs to have an email account with a public email provider, and needs to know the public information related to \name, e.g., the email addresses of \name.



\paragraphb{\bf No need to share secrets:} To ensure availability and unobservability, several  circumvention tools need to share some secret
information with their users, in order to initiate  the circumvented a connection\cite{tor-bridge,collage,infranet,Karlin2011}.
This is a significant limitation, as keeping such information  secret from the censorship authorities is  a hard problem, and the disclosure of such secret information breaks their unobservability and availability promises.
A \name user does not require to obtain any secret information from the \name server.
%In order to use \name, a user only needs to know the publicly available email address of the \name system. The public disclosure of this email address does not degrade the unobservability and availability promises of \name.


\begin{comment}
\paragraph{\bf User anonymity:} A \name client communicates with the \name system through email messages that are delivered by the client's public email provider, e.g., Gmail, Yahoo! Mail, etc. As a result, the \name server is not able to link a user's public email address to her IP address, hence, to her identity.



%\subsection{Comparison with literature}\label{sec:comparison}

Table~\ref{tab:comparison} compares some of the key features of \name with a number of popular/recent circumvention systems.

\begin{table*}[tbp]
\centering
\caption{Comparing some key features of \name with popular/recent circumvention systems}
\begin{tabular}{|l|l|c|l|c|}
\hline
System & Ease of deployment & Reliance on shared secret & Unobservability & Anonymity \\ \hline \hline
Infranet\cite{infranet} & Needs collaborating end-hosts & Yes & Bound to the secrecy of the shared secret& No \\ \hline
Collage\cite{collage} & Standalone & Yes & Bound to the secrecy of the shared secret & No \\ \hline
Tor~\cite{onion-routing} & Needs collaborating servers & No & no & Yes \\ \hline
Tor with bridges \cite{tor-bridge} & Needs collaborating servers and hosts & Yes & Bound to the secrecy of the shared secret & Yes \\ \hline
Telex~\cite{Wustrow2011}  & Needs collaborating ISPs & No & yes & No \\ \hline
Cirripede~\cite{Houmansadr2011a}  & Needs collaborating ISPs & No & Yes & No \\ \hline \hline
\name & Standalone & No & Yes & Yes \\ \hline
\end{tabular}
\label{tab:comparison}
\end{table*}

\end{comment}




\if 0
\begin{table*}
\centering
\caption{Comparison  \name with popular circumvention approaches}
 \begin{tabular}{|l|c|c|c|c|}
\hline
Circumvention System & Unobservability& Availability & Ease of deployment & Reliance on shared secrets

System & Infranet~\cite{infranet} and Collage~\cite{collage} & Tor~\cite{onion-routing} & Tor with bridges \cite{tor-bridge}& In-network approaches \cite{Wustrow2011,Karlin2011,Houmansadr2011a}\\

Need for pre-shared secret information\\
Possibility of getting blocked\\
Reliance on third parties\\

 \name a& A& \\
\hline
 \end{tabular}
\label{tab:comparison}
\end{table*}

\fi



%\subsubsection{Security evlauation}






==> files/implementation.tex <==
\section{Prototype Implementation} \label{sec:implementation}
%and measurements


We have  prototyped the \name circumvention system and measured its performance.

\subsection{Server implementation}

We implement the \name server on a Linux machine. The machine runs \textit{Ubuntu 10.04 LTS} and has a 2 GHz quad-core CPU and 4 GB of memory.
We run  Postfix\footnote{\url{http://www.postfix.org/}}, a simple email server
that supports basic functions. Postfix listens for new emails targeted to
the {\tt register@sweet.org} and {\tt tunnel@sweet.org} email addresses. Postfix stores the received emails into designated file directories that are continuously watched by the converter and registration agent components  of \name server.
Each stored email has a unique name, concatenating the email id of its corresponding client and an increasing counter.
The converter agent is a simple Python-based program that runs in the background and continuously checks the folder for new emails. The converter also converts proxied packets, passed by \name's proxy, into email messages and sends them to their intended clients.
For the proxy agent, we use Squid\footnote{\url{http://www.squid-cache.org/}} as our HTTP proxy and Suttree\footnote{\url{http://suttree.com/code/proxy/}} as our SOCKS proxy.
Squid runs on a local port and  listens for connections from the converter component.



\subsection{Client implementation}
We implement both protocol-based and webmail-based versions of the \name client.

\paragraphb{Protocol-based design} The client prototype is built on a desktop machine, running \textit{Linux Ubuntu 10.04 TLS}.
We set up a web browser to use the local port "localhost:9034" as the SOCKS/HTTP proxy. The converter component of \name client is a simple python script that listens on port 9034
for connections, e.g., from our web browser. Finally, we implement the email agent of \name client
using \textit{Fetchmail}\footnote{\url{http://www.fetchmail.info/}}, a popular client software for sending and retrieval of emails through email protocols. We generate a free Gmail account and configure Fetchmail to receive emails through IMAP\footnote{\url{https://mail.google.com/support/bin/answer.py?answer=78799}} and POP3\footnote{\url{https://mail.google.com/support/bin/answer.py?answer=13287}} servers of Gmail, and to send emails through the SMTP server of Gmail\footnote{\url{https://mail.google.com/support/bin/answer.py?answer=78799}}.
Note that our design does not rely on Gmail, and the  client software can be set up with any email account.

\paragraphb{Webmail-based design}
Our webmail-based implementation also runs on \textit{Linux Ubuntu 10.04 TLS}.
Our webmail-based implementation uses a Google Chrome browser for making connections through \name, configured to use the local port of "localhost:9034" as a proxy. Also, the webmail-based design uses the same  converter component as the one used in the protocol-based prototype.

We prototype the web-based email agent  by running a \textit{UserScript}\footnote{\url{http://userscripts.org/}} inside the Mozilla Firefox\footnote{\url{http://www.mozilla.org/en-US/firefox/new/}} web browser.
More specifically, we install a Firefox  extension, called \textit{Greasemonkey}\footnote{\url{https://addons.mozilla.org/en-US/firefox/addon/greasemonkey/}}, that allows a user to run her own JavaScript, i.e., Userscript, while browsing certain destinations. We write a UserScript that runs in Gmail's webmail interface and listens for the receipt of new email messages. Our UserScript saves new emails in a local directory, which is watched by the converter component. Note that the Firefox browser is directly connected to the Internet and does not use any proxies (user needs to use the configured Chrome browser to surf the web through \name).

\section{Evaluation}  \label{sec:eval}

We evaluate \name using our prototype implementation, described in Section~\ref{sec:implementation}.

%We browse  many websites using our protocol-based and webmail-based \name clients
%and measure the time that \name browser (Chrome browser) takes to render the website.

\subsection{Performance}

We use Gmail as the oblivious mail provider in our experiments. Our \name server is located in Urbana, IL, resulting in approximately 2000 miles of geographic distance between the \name server and Gmail's email server (we locate Gmail's location from its IP address).
Figure~\ref{fig:mailtrans} shows the CDF of the time that  a \name email (carrying the tunnelled traffic) sent by a \name client  takes to reach our \name server (the reverse path takes a similar time).
As the  figure shows,  around 90\% of \name emails take less than 3 seconds to reach the \name server, which is very promising considering the high data capacity of these email messages.
Note that based on our measurements,  most of this delay comes from email handling (e.g, spam checks, making SMTP connections, etc.) performed by the oblivious mail provider (Gmail in our experiments), but not from the network latency (the network latency and client latency constitute only tens of milliseconds of the total latency). As a result, the latency would be very similar for users with an even longer geographical distance from the oblivious mail server.

\begin{figure}
\centering
 \includegraphics[width= 0.8\columnwidth]{figs/impl/mailTrans}
\caption{The CDF of the time that a \name email takes to travel from the \name client to the \name server (100 runs).}
\label{fig:mailtrans}
\end{figure}


\paragraphb{Client registration}
Before being able to request data from Internet destinations, a user needs to be registered by the \name server. Figure~\ref{fig:cdf_socks} shows the time taken to exchange registration messages between a client and the \name server.
Note that the client registration needs to be performed \textit{only once} for a long period of time. The figure shows that more than 90\% of registrations establish in less than 8 seconds (with an average of 6.4 seconds).


%
%Before being able to request data from Internet destinations, a connection needs to be established between the client and the proxy server of \name.  Figure~\ref{fig:cdf_socks} shows the time that takes for client's web browser to establish a proxy connection with the proxy agent of \name server. Note that the proxy connection needs to be performed \textit{only once} for a long period of time, e.g., the client can keep a proxy connection open for long periods and use that one connection to request data from many destinations. The figure shows that more than 90\% of proxy connections establish in less than 8 seconds. The  average time for proxy establishment is 6.4 seconds.



\begin{figure}
\centering
 \includegraphics[width= 0.8\columnwidth]{figs/impl/cdf_socks}
\caption{The CDF distribution of the registration time. }
\label{fig:cdf_socks}
\end{figure}


We use two metrics to evaluate the latency performance of \name in browsing websites: the \emph{time to the first appearance (TFA)} and
the \emph{total browsing time (TBT)}. As described by its name, the TFA is the time taken to receive the first response from a requested web destination. The TFA is an important metric in measuring  user convenience during web browsing.  For instance, suppose that a client requests a  URL, e.g.,  \url{http://www.cnn.com/some_news.html}. By the TFA time the client receives the first HTTP RESPONSE(s) from the destination, which include the URL's text parts (perhaps the news article) along with the URLs of other objects on that page, e.g., images, ads hosted by other websites, etc. At this time the client can start reading the received portion of the website (e.g., the news article), while her browser sends requests for other objects on that webpage.
On the other hand, the total browsing time (TBT) is the time after which the browser finishes fetching all of the objects in the requested URL.


%We perform two types of experiments to evaluate the web browsing experience using \name. In the first experiment, namely \emph{HTML-download} experiment,  we use the \name client to download a web page, while ignoring the objects in the webpage. In the second experiment, called \emph{web-browse} experiment, we use the \name client to browse a web page, i.e., \name browser sends HTTP requests for all of the objects of that web page. We next report the results of the experiments. The HTML-download experiments represents web pages that are less-interactive, e.g., search results, and news pages, while the web-browse experiments represent web pages that need more interaction with a browser, e.g., login pages and pages with AJAX-based objects.

Using our prototype we measure the end-to-end web browsing latency for the client to reach different web destinations. Figure~\ref{fig:1stround_each} shows the time to the first appearance (TFA) using \name for the top 10 web URLs from  Alexa's most-visited sites ranking \cite{alexa}. As can be seen, the median of the TFA is about 5 seconds across all experiments, which is very promising to user convenience.




\begin{figure}
\centering
 \includegraphics[width= 1\columnwidth]{figs/impl/mb/1stround_each}
\caption{The  CDF of   the time to the first appearance (TFA) of \name.}
\label{fig:1stround_each}
\end{figure}


\if 0
\subsubsection{Time to the first appearance (TFA)}

%We measure the delay performance of our prototype implementation for web browsing. In the first set of experiments, we use \name to browse the text part of the webpages, e.g., the browser does not request the non-text objects of a webpage.

We use \name to download the top 10 web URLs from  Alexa's most visited sites ranking \cite{alexa} (each URL is requested for 50 times). Figure~\ref{fig:wget_each_all} shows the CDF of the time to download these pages using \name, where each web site is browsed for 50 times. The figure also shows the average CDF. As can be seen  \%60 of all requests are finished in less than 10 seconds and \%90 of all requests are completed in less than 15 seconds. In particular, a Google search result is returned in less than 8 seconds in \%90 of all runs.


\begin{figure}
\centering
 \includegraphics[width= 1\columnwidth]{figs/impl/wget/wget_each_all}
\caption{The  CDF of the HTML-download experiment through \name.}
\label{fig:wget_each_all}
\end{figure}

\fi

\begin{comment}
As can be seen, .... google. Figure~\ref{fig:normal-wget-each} shows the time to download with a direct conncetion and without using our system. As one could expect, the use of \name increases the time for web browsing as compared to a direct connection, however, we see that the extra latency is reasonable and provides a convenient  web browsing experience. Figure~\ref{fig:2_wget_all} compares the CDF of time to download for a direct connection and using \name.


\begin{figure}
\centering
 \includegraphics[width= 0.5\textwidth]{figs/impl/wget/normal_wget_each}
\caption{The CDF of the time to download a website using a direct connect from Alexa's global top 10 ranking (only the text part).}
\label{fig:normal-wget-each}
\end{figure}

\begin{figure}
\centering
 \includegraphics[width= 0.5\textwidth]{figs/impl/wget/DirectVsSWEET}
\caption{The CDF of the time to download for all websites (500 runs).}
\label{fig:2_wget_all}
\end{figure}

\end{comment}



\begin{comment}
\begin{figure}
\centering
 \includegraphics[width= 0.5\textwidth]{figs/impl/curl_google}
\caption{The CDF of the time to receive  a search result from Google search engine (100 runs).}
\label{fig:curlgoogle}
\end{figure}


\begin{figure}
\centering
 \includegraphics[width= 0.5\textwidth]{figs/impl/curl_20}
\caption{The CDF of the time to download one of Alexa's global top 20 websites (200 runs).}
\label{fig:curl20}
\end{figure}
\end{comment}



On the other hand, Figure~\ref{fig:mb_each} shows the total browsing time (TBT) using \name for the same set of destinations (50 runs for each website).
As can be seen, the  destinations that contain more web objects (e.g., yahoo and linkedin) take more time to get completely fetched (note that after the TFA time the user can start reading the webpage until all of the objects are received). We also run similar experiments through the popular  Tor~\cite{onion-routing} anonymous network to compare its latency performance with \name.
Figure~\ref{fig:mb_SWEETVsTor} compares the cumulative time CDF for \name and Tor systems. As expected, our simple implementation of \name takes more time than Tor to browse a web page, however, it provides a sufficient performance for normal web browsing. This is in particular significant considering the strong \emph{availability} of \name compared to other circumvention systems, as discussed in this paper.  Additionally, we believe that further optimizations on \name server's proxy (like those implemented by Tor exit nodes) will further improve the latency of \name.
 Our techniques are also amenable to standard methods to improve web
latency, such as plugin-based caching and compression, which can make
web browsing tolerable in high delay environments \cite{conf/www/ChenHTS11}.

\begin{figure}[t]
\centering
 \includegraphics[width= 1\columnwidth]{figs/impl/mb/mb_each}
\caption{The  CDF of the TBT time using \name.}
\label{fig:mb_each}
\end{figure}

\begin{figure}
\centering
 \includegraphics[width= 1\columnwidth]{figs/impl/mb/mb_SWEETVsTor}
\caption{Comparing the average latency of \name and Tor.}
\label{fig:mb_SWEETVsTor}
\end{figure}




\if 0
\paragraph{Total browsing time (TBT)}

While the HTML web download is enough for many Internet browsing activities (e.g., google search, news reading, etc.), in several cases the browser needs to maintain an interactive connection with a web destination. Examples for such cases are the login-based websites, and  posting on social networks (e.g., twitter.com, facebook.com). In addition, some web objects, like JAVA and  AJAX, rely on maintaining a live TCP connection with a user's browser. In the second set of our experiments, we evaluate a full browsing experience through \name. Figure~\ref{fig:mb_each} shows the CDF of the times to complete browsing a web page using \name. To compare our results with the popular Tor~\cite{onion-routing} anonymous network, we also run similar experiments through Tor, as shown in Figure~\ref{fig:tor_mb_each}. Also, Figure~\ref{fig:mb_SWEETVsTor} compares the cumulative time CDF for \name and Tor systems. As expected, our simple implementation of \name takes more time than Tor to browse a web page, however, it provides a sufficient performance for normal web browsing. This is in particular significant considering the strong \emph{availability} of \name compared to other circumvention systems, as discussed in this paper.  Additionally, we believe that further optimizations on \name server's proxy (like those implemented by Tor exit nodes) will further improve the latency of \name.


%and Figure~\ref{fig:normal_mb_each}  shows the same results with a direct connection without using \name. Also, Figure~\ref{} shows the same results using the Tor~\cite{onion-routing} anonymous network. As can be seen, ..... Figure~\ref{fig:2_mb_all} compares the total CDF for the three cases.


\begin{figure}[t]
\centering
 \includegraphics[width= 1\columnwidth]{figs/impl/mb/mb_each}
\caption{The time CDF of the TBT time using \name.}
\label{fig:mb_each}
\end{figure}

\begin{figure}[t]
\centering
 \includegraphics[width= 1\columnwidth]{figs/impl/mb/tor_mb_each}
\caption{The time CDF of the web-browse experiment through Tor.}
\label{fig:tor_mb_each}
\end{figure}

%\begin{figure}
%\centering
% \includegraphics[width= 0.5\textwidth]{figs/impl/mb/normal_mb_each}
%\caption{The CDF of the time to download one of Alexa's global top 10 websites (50 runs for each website).}
%\label{fig:normal_mb_each}
%\end{figure}

\begin{figure}
\centering
 \includegraphics[width= 1\columnwidth]{figs/impl/mb/mb_SWEETVsTor}
\caption{The average time CDF of the web-browse experiment through \name and Tor systems.}
\label{fig:mb_SWEETVsTor}
\end{figure}




\fi



\begin{comment}

Finally, figure~\ref{fig:cdf_data} illustrates the CDF of the time that the client browser takes to download a requested website through \name (100 runs). As can be seen, the average delay is around 6.46 seconds, which is comparable to that of other  censorship circumvention systems \cite{collage,infranet,onion-routing}.
Note that based on our experiments downloading different-size websites (ranging from one KB to tens of KB), the size of the website only slightly influences the total download time, since the total delay is dominated by the email transmission times, not the size of the requested website.

\begin{figure*}
\centering
 \includegraphics[width= 0.5\textwidth]{figs/impl/cdf_data}
\caption{The CDF distribution of the time to download a website using the protocol-based client of \name (100 experiments).}
\label{fig:cdf_data}
\end{figure*}

We also performed similar measurement using our webmail-based prototype. Figure~\ref{fig:cdf_data_web} shows the time to download a website through our webmail-based client prototype. The average download time is around 7.46 seconds.

\begin{figure*}
\centering
 \includegraphics[width= 0.5\textwidth]{figs/impl/web}
\caption{The CDF distribution of the time to download a website using the webmail-based client of \name (100 experiments).}
\label{fig:cdf_data_web}
\end{figure*}

%have different  implementation (1) downloading the webpage (2) socks proxy (3) the web-based implementation for gmail



%measure the connection delays for different types of connection (and compare it with other curcumvention systems like Tor)


\end{comment}


\subsection{Traffic analysis}\label{sec:trafanal}

%We argued in Section~\ref{sec:enc} that unobservability might only be a concern to specific citizens, e.g., political activists. 
A powerful censor can perform traffic analysis to detect the use of \name, e.g., by comparing a user's email communications with that of a typical email user.  As a result, a \name user who is concerned about unobservability needs to ensure that her \name email communications mimic that of a normal user (as discussed in Section~\ref{sec:enc}, a user who does not fear reprisal from her
government might opt to ignore unobservability in order to gain a higher communication bandwidth). It should be mentioned that such traffic analysis is expensive for censors considering the large volume of email communications; it is estimated\footnote{\url{http://royal.pingdom.com/2011/01/12/internet-2010-in-numbers/}} that 294 billion email messages were sent per day in 2011.

Figure~\ref{fig:num} shows the number of emails sent and received by a \name client to browse different websites. We observe that for any particular website the number of emails does not change at different runs. As can be seen, most of the web sites finish in less than three \name emails in each direction. The exception is the Yahoo web page as it contains many web objects, each hosted by different URLs (note that the number of email messages affects the latency performance only \emph{sub-linearly}, since some emails are sent and received simultaneously.).   Also, the average number in each way of a connection is about 4 emails.
A recent study \cite{email-stat} on email statistics predicts that an average user will send 35 emails and will receive 75 emails per day in 2012 (the study predicts the numbers to increase annually). In addition, membership in mailing lists\footnote{\url{http://gcc.gnu.org/lists.html}} and Internet groups\footnote{\url{http://groups.yahoo.com}}\footnote{\url{http://groups.google.com}} is popular among Internet users, producing  even more emails by normal email users. As an indication of the popularity of such services, Yahoo in 2010  announced\footnote{\url{http://www.eweek.com/c/a/Search-Engines/Yahoo-Refreshes-Upgrades-Some-Products-775120/}} that  115 million unique users are collectively members of more than 10 million Yahoo Groups. Based on the mentioned statistics,  we estimate that a conservative \name user can perform 35-70 web downloads per day, or make 10-20 interactive web connections, while ensuring unobservability of \name usage. Once again, as discussed in Section~\ref{sec:enc}, we argue that unobservability is a concern only to special citizens; hence, we believe  that  normal citizens would use \name ignoring the possibilities of traffic analysis by a censor.

\begin{figure}
\centering
 \includegraphics[width= 1\columnwidth]{figs/impl/mb/rcv_sd}
\caption{The number of emails sent and received by a \name client to get one of the websites from Alexa's top ten ranking.}
\label{fig:num}
\end{figure}

\begin{comment}
\begin{table}
\centering
\caption{The number of emails sent and received by a \name client to get one of the websites from Alexa's top ten ranking.}
\begin{tabular}{|c|c|c|}
\hline
Website                 &             Sent            &Received\\\hline
www.google.com            &2                  &2\\
www.facebook.com        &3                  &3\\
www.youtube.com          &6                  &5\\
www.yahoo.com             &7                  &7\\
www.baidu.com              &3                  &2\\
www.wikipedia.org          &5                  &5\\
login.live.com                 &2                  &2\\
www.twitter.com                     &3                  &5\\
www.linkedin.com                  &4                  &6\\
www.amazon.com           &5                  &5\\\hline
Average & 4 & 4.2 \\\hline
\end{tabular}\label{tab:num}
\end{table}
\end{comment}


%%
%%Another possibility for  traffic analysis is to monitor the density of the email messages. In \name emails are sent and received in bursts





==> files/introduction.tex <==
\section{Introduction}
\label{sec:introduction}

%First, show that the problem of censorship is very severe.

Today's Internet provides users with an environment to freely communicate, and
to exchange ideas and information with others from around the world.  However,
free communication continues to threaten repressive regimes, as the open
circulation of information and speech among their citizens can pose serious
threats to their existence. Recent unrest in the middle east demonstrates that
the Internet can be widely used by citizens under these regimes as a very
powerful tool to spread censored news and information, inspire dissent, and
organize events and protests.  As a result, repressive regimes extensively
monitor their citizens'    access to the Internet and restrict open access to
public networks  \cite{zit03} by  using different technologies, ranging from
simple IP address blocking (e.g., through access control lists) and DNS
hijacking to more complicated and resource-intensive Deep Packet Inspection
(DPI) \cite{gifc:07,Leberknight2010}.
%Users found to be trying to evade the censor's restrictions can be in the utmost danger, facing financial fines, imprisonment, and even death.

%a%The modern Internet was born in the 1990s to provide users from around the world with an environment to freely communicate, and exchange ideas and information with the rest of the world. This is unpleasant to repressive regimes as the free circulation of information and speech among their citizens can pose serious threats to their benefits and even their existence. Recent unrest in the middle east show that the Internet is widely used by the citizens under oppressive regimes as a very power tool to spread the censored news and information, organize different events and protests. As a result, repressive regimes extensively monitor their citizens' access to the Internet and restrict the open access to the Internet \cite{zit03} by using different technologies and tools.  The censors use different censorship technologies ranging from simple IP-address blocking and DNS hijacking to the more complicated and resource-intensive Deep Packet Inspection (DPI) techniques \cite{gifc:07,Leberknight2010}. A user detected to be trying to evade the censor's restrictions can face drastic life-threatening consequences, e.g., financial fines or imprisonment, depending on the level of violation.

%Second, introduce the recent progress on anti-censorship.
With the use of censorship technologies, a number of different systems were developed to retain the openness of the Internet for the users living under repressive regimes \cite{freenet,ultrasurf,Psiphon,dingledine:sec04,anonymizer}. These systems are composed of an ensemble of network hosts and use different computer and networking technologies to evade the monitoring and blocking performed by the censors. The earliest circumvention tools are HTTP proxies \cite{anonymizer,freenet,dynaweb}  that simply intercept and manipulate a client's HTTP requests, defeating IP address blocking and DNS hijacking techniques. The use of more advanced censorship technologies such as deep packet inspection~\cite{gifc:07,ClaytonMW06},  rendered the use of HTTP proxies ineffective for circumvention. % in circumventing censorship, as the censors were able to monitor the packet contents.
This led to the advent of more advanced circumvention tools such as Ultrasurf~\cite{ultrasurf} and Psiphon~\cite{Psiphon}, designed to evade content filtering performed by the more advanced censors.
%More recently, several research has been proposed that are based on some capabilities built inside the Internet to help evade the censorship \cite{Karlin2011, Wustrow2011,Houmansadr2011a}.
In addition to special-purpose anti-censorship systems,  many users have been using anonymity systems as effective tools to evade Internet censorship \cite{Leberknight2010,gifc:07}. These systems are designed to hide a user's activity over the Internet,  which can also help to evade Internet censorship since the censor will not be able to determine the network destination of a user's
traffic. Multiple designs have been proposed for anonymity systems, including the onion routing~\cite{onion-routing} and mix networks~\cite{chaum:mixnet}.


While these circumvention tools have helped, they face several challenges that
prevent them from being a good choice for a longer-term solution to Internet
censorship.
We believe that the biggest challenge to existing circumvention systems is their lack of \emph{availability}, meaning that a censor can
disrupt  their service frequently or even disable them completely \cite{Sovran2008,McCoy2011,Feamster03,springerlink:10.1007/978-3-642-13122-6_29,McLachlan2009}.
The common reason leading to the mentioned lack of availability is that the network traffic made by these systems can be distinguished from regular Internet traffic by censors, i.e., such systems are not \emph{unobservable}. This enables censors to disrupt/block the communications made by their citizens to such circumvention systems.
For example, the popular Tor \cite{dingledine:sec04}  network works by having users connect to an ensemble of nodes with public IP addresses, which proxy the user's traffic to the requested, censored destinations. This public knowledge about Tor's IP addresses, which is required to make Tor usable by users globally, can be/is used by censors to block their citizens from accessing Tor \cite{china-tor,tor-blocked}.
%The lack of unobservability can be used by a censor to block access to the service, e.g., filtering the known IP addresses of the Tor nodes in the mentioned example.
%This can also be used to locate and prosecute identified users of such systems, though this rarely happens for normal citizens, as discussed later in this paper.
To improve their availability, recent proposals for circumvention aim to make their traffic unobservable from censors \cite{infranet,collage, tor-bridge,Karlin2011, Wustrow2011,Houmansadr2011a}.
Several designs \cite{infranet,collage, tor-bridge} seek unobservability by sharing secret information with their clients, which are not known to censors.
For instance, the Tor network has recently adopted the use of \emph{Tor Bridges}, a set of volunteer nodes connecting clients to the Tor network, whose IP addresses are selectively distributed among Tor users by Tor. Unfortunately, this approach poses another challenge \cite{springerlink:10.1007/978-3-642-13122-6_29,McLachlan2009}, which is sharing such secret information only with real users in a scalable manner such that it is not disclosed to the censors pretending to be users.
%One example is the Infranet
%system \cite{infranet} that requires a    secret key and also a secret web URL
%to be provided to the client in advance of the usage.  Relying on secret
%information makes such systems prone to   different issues; first, the
%distribution of the secret information to the users is  challenging and faces
%scaling challenges \cite{springerlink:10.1007/978-3-642-13122-6_29}.  Second,
%it is difficult to keep the secret information secret from the censor, as the
%censor can play the role of a user to obtain such information
%\cite{McLachlan2009}.  Having the secret information exposed to the censor can
%result in blocking the system, identifying the system's users, or even
%disclosing the past  activity of the identified users \cite{McLachlan2009}.
A more recent approach in designing unobservable, hence highly-available, circumvention systems is to integrate
 censorship circumvention with the Internet infrastructure \cite{Karlin2011, Wustrow2011,Houmansadr2011a,lap}.  Telex~\cite{Wustrow2011},
Cirripede~\cite{Houmansadr2011a}, and LAP~\cite{lap} are example designs that suggest modifications to Internet infrastructure, e.g., routing decisions, in order to hide users'  circumvented traffic from their monitoring censors.
Even though such systems provide better availability promises, compared to traditional circumvention, their deployment requires substantial modifications to ISP networks, requiring
cooperation from ISP operators and/or network
equipment vendors, presenting a substantial deployment
challenge.




%a%Third, point out the limitations of these solutions: require support of ISP.
%a% Even though the mentioned circumvention tools have helped many users during the last decade to evade the Internet censorship, they  face
%a% several challenges that prevent any of them to be considered as a reliable and long-term circumvention tool.
%a% Many of the circumvention tools lack the \textit{unobservability} property, meaning that a sensor can detect
 %a% whether a user is using such systems \cite{anonymizer,dingledine:sec04, more}.
 %a% As an example, since the identity of the Tor nodes \cite{dingledine:sec04} are publicized,  a censor can easily identify the users connected to the Tor network's entry nodes.
%a% The lack of unobservability can be used by a censor to either block the access to the service, or even penalize the identified users of such systems.
%a% In order to provide unobservability, some circumvention techniques share some secret information with their users, e.g., secret keys or secret design knowledge, so that an entity not having such secret information will not able to either use the system or identify the users of such systems.
%a% An example of such schemes is the Infranet system \cite{infranet} that requires a secret key and also a secret web URL to be provided to the client in advance to the usage.
%a% Relying on the secrecy of a  secret information makes such systems prone to different issues; first, the distribution of the secret information to the users is challenging and is not very scalable \cite{springerlink:10.1007/978-3-642-13122-6_29}. Second, it is hard to keep the secret information secret from the censor as the censor can play the role of a user to obtain such information \cite{McLachlan2009}. Having the secret information exposed to the censor can result in blocking the system, identifying the system's users, or even disclosing the past activity of the identified users \cite{McLachlan2009}. More recently, several techniques suggest to build censorship circumvention within the Internet, i.e., by modifying a number of the Internet routers running inside the uncensored regions \cite{Karlin2011, Wustrow2011,Houmansadr2011a}. Such systems provide higher degrees of unobservability, as compared to the previous approaches, however, the need for collaboration from ISPs is a challenge for the real-world implementation of such services.


%, highlight our solution.
In this paper, we design and implement \name, a censorship circumvention system that  provides high availability by leveraging the openness of email communications. Figure~\ref{fig:main} shows the main architecture of \name.  A \name  client, confined by a censoring ISP,   tunnels its network traffic with  blocked destinations inside a series of email messages that are exchanged between the client and an email server operated by \name's server. The \name server, then, acts as an Internet proxy \cite{RFC1928} for the client by proxying the encapsulated traffic to blocked Internet destinations.
The \name client uses an oblivious, public mail provider (e.g., Gmail, Hotmail, etc.) to exchange the encapsulating emails, rendering standard email filtering mechanisms ineffective in identifying/blocking \name-related emails. More specifically, to use \name for circumvention a client creates an email account with \emph{any} public email provider (e.g., Gmail, Hotmail) and obtains \name's client software from an out-of-bound channel (similar to other circumvention systems). The user configures the installed \name software  to use her public email account, which sends/receives  encapsulating emails messages on behalf of the user to/from the publicly known email address of \name, e.g., {\tt tunnel@sweet.org}.
Note that there is no need for the user to  obtain any secret information, secret key, or secret design information  in order to use \name.
%The use of encrypted emails protects an optional protection, as discussed in the paper.


\begin{figure*}
\centering
 \includegraphics[width= 0.5\linewidth]{figs/mailmynet_main}
\caption{Overall architecture of \name.}
\label{fig:main}
\end{figure*}

\name provides several key advantages as compared to the existing circumvention systems. First, since email is an essential service
in today's  Internet it is very unlikely that a censorship authority will block \textit{all} email communications to the outside world, due to different financial and political reasons. This, along the fact that \name can be reached through \emph{any} email service, provides a high degree of \emph{availability} for \name since a censor will need to block all email traffic to the Internet in order to block \name.
Second, by using encrypted email messages \name is highly unobservable from the censors.
Third, the real-world deployment of \name does not require cooperation of any third-party entity,
e.g., an ISP,  a web destination, or even an specific email provider.
Finally, unlike several recent proposals~\cite{infranet, collage,Karlin2011, tor-bridge} a \name user does not have to obtain any secret information in order to use \name, providing high  user convenience and ensuring the security and privacy of the user.

%We thoroughly compare our \name design with popular circumvention approaches in Section~\ref{sec:discussions}.

%Finally, as we discuss in Section~\ref{sec:enc} usage unobservability is a desired feature for \emph{some} users, e.g., a political activist~\footnote{We argue that unobservability is not a concern for normal citizens, hence we provide it as an option to the user.}. The encrypted version of \name provides plausible unobservability, as discussed in the paper.


In fact, the high availability of \name comes for the price of higher, but bearable, communication latencies. Figure~\ref{fig:availability} compares \name with several popular circumvention systems regarding their availability and communication latency. As our measurements in Section~\ref{sec:eval} show, \name provides communication latencies that are convenient for latency-sensitive activities like web browsing (i.e., few seconds). Such additional, tolerable latency of \name comes with the bonus of better availability, as discussed in Section~\ref{sec:availability}.

\begin{figure}
\centering
 \includegraphics[width= \linewidth]{figs/availability}
\caption{Comparing availability and communication latency of several circumvention systems.}
\label{fig:availability}
\end{figure}




%Second, considering that most email providers support encryption of email communications (either though HTTPS access through a web-based interface or encrypted SMTP, IMAP, and POP protocols), a user can disguise her use of the \name system. This provides plausible unobservability for \name, a key feature missing in many circumvention systems.

We have built a prototype implementation for the \name system and evaluated its performance.
We have also prototyped two different designs for \name's client software, as proposed in this paper. The first client design uses email protocols, e.g., POP3 and SMTP, to communicate with the
\name system, and our second design is based on using the webmail interface.
Our measurements show that a \name client is able to browse regular-sized web destinations
with download times in the order of couple of seconds.

In summary, this paper makes the following main contributions: i) we propose a novel infrastructure for censorship circumvention, \name, which provides high availability, a feature missing in practical circumvention systems; ii) we develop two prototype implementations for \name (one using webmail and the other using email exchange protocols) that allow the use of nearly all email providers by \name clients; and, iii) we show the feasibility of \name for practical censorship circumvention by measuring the communication latency of \name for web browsing using our prototype implementation.

%use email as a widely used service which is not blockable
%no need for collaboration
%use of encryption provides unobservability
%no need for secret info


%Fifth, roadmap.
The rest of this paper is organized as follows; in Section~\ref{sec:related}, we provide some background information and discuss the related work on censorship circumvention.
In Section~\ref{sec:model}, we reviews our threat model. We provide the detailed description of the proposed circumvention system, \name,  in Section~\ref{sec:scheme}. We discuss \name's censorship features, including its availability,  in Section~\ref{sec:discussions} and compare it with the literature. Our prototype implementation and evaluations are
presented in Sections~\ref{sec:implementation} and \ref{sec:eval}, respectively. Finally, we conclude the paper in Section~\ref{sec:conclusions}.




\if 0
\section{Background and related work}
\label{sec:backgroundrw}

\subsection{Email communication protocols}

Electronic mail, commonly referred to as email~\cite{RFC2045,RFC2049}, is a widely used method of exchanging digital messages between users
of computer networks. Today's modern email systems are based on a \textit{store-and-forward} model, such that an email server is responsible for receiving and storing a user's email messages, without the need for the user to be online during the email's transmission. The stored email messages can be retrieved at any time upon the user's request.
Email is capable of carrying multi-media content attachments \cite{RFC2045,RFC2049}. Depending on the email provider of the sender and the receiver, an email can carry attachments of tens to hundreds of megabytes.

A number of Internet protocols are designed for  Internet users to communicate with email servers and to send and receive email messages. In particular, the Internet Message Access Protocol (IMAP) \cite{RFC3501} and the Post Office Protocol (POP) \cite{RFC1939} are two popular protocols for email retrieval, that are supported by almost every modern email client and email server.   On the other hand, the Simple Mail Transfer Protocol (SMTP) \cite{RFC5321} is the standard for sending email messages. Client email software uses the SMTP protocol to send email to an email server, and uses any of the IMAP or POP protocols for retrieving emails from the email server.

As an alternative to the use of email protocols by client software to exchange emails, many email providers provide users a web interface to send and receive emails, sometimes referred to as {\em webmail}. One key advantage of webmail over desktop email clients is the ability to exchange wherever there is a browser. The downside, however, is the need for Internet access to read previously received emails (though Gmail now provides support for offline access to emails).

%some usage statistics

\subsection{Internet proxies}\label{sec:proxy}
In computer networks, a proxy server is a server that acts as an intermediary for network connections from clients to servers. More specifically, instead of directly connecting to a destination, a client requests the proxy server to access that destination on behalf of the client. There are different incentives for using a network proxy, including evasion of Internet censorship, providing anonymity, speeding up a connection, bypassing security controls, etc.

While there are a number of different protocols used to form proxy-based communication, two protocols are among the most widely
%Among different proxy protocols that are designed two protocols are most widely
used: the HTTP~\cite{RFC2616}  proxy  and the SOCKS proxy \cite{RFC1928} protocols.
SOCKS is an Internet protocol that is used to route data packets between network entities using a proxy \cite{RFC1928}.
SOCKS works at the session layer of the Open Systems Interconnection (OSI) model.
On the other hand, HTTP proxies work at the application-layer of the OSI model and
establish HTTP connections to the requested server on behalf of clients.

%An alternative scheme to proxy traffic is with application-layer schemes,
%for example by using an HTTP proxy.
%works
%An alternative protocol is the HTTP proxy that works on the application layer by receiving  HTTP web requests form the client and establishing an HTTP connection to the requested server.

The SOCKS and HTTP proxies have several advantages and disadvantages compared to  each other, making them suitable for different applications.
The main advantage of the SOCKS proxy over the HTTP proxy is that  the HTTP proxy is designed  to proxy only the HTTP Internet traffic, whereas a SOCKS proxy can route any IP Internet traffic, including both TCP- and UDP-based traffic.
%In particular, the SOCKS proxy can route all TCP-based communications, as well as the UDP Internet traffic.
Another advantage is that the latest version of SOCKS (SOCKS5~\cite{RFC1928})  provides
user authentication \cite{RFC1929}, allowing restriction of the use of the proxy
service only to authorized users.
%As another advantage over  the HTTP proxy,  the latest version of the SOCKS proxy, SOCKS5, provides user authentication to restrict the use of the proxy service only to the authorized users.
In contrast,  HTTP proxies can use  pre-fetching of web content and other HTTP-layer optimizations to speed up the proxied HTTP connection. Web caching~\cite{caching} can be used as an effective technique to reduce the latency and bandwidth constraints of the  proxy server for both SOCKS and HTTP proxies.

The use of SOCKS has been adopted by a number of Internet services. For example, the popular Tor~\cite{onion-routing} anonymous communication network deploys a SOCKS proxy at its client software to tunnel a client's Internet traffic to the Tor network proxies. Also, SOCKS proxies have been widely used as  Internet proxies to evade censorship circumvention systems. On the other hand, HTTP proxies have been widely used in web services.

%In this paper, we use the SOCKS proxy in the design of \name, our anti-censorship system, to establish a network connection between a censored user and her requested blocked web destination. This SOCKS-based connection is tunneled within email communications among the user and \name's server.


%%Question:Move related work as background section??


\subsection{Censorship circumvention}

\fi


\section{Related work}\label{sec:related}
As a result of extensive censorship of the Internet by repressive regimes,
affected citizens have been looking for effective tools to
%evade such filtering and gain an
gain unrestricted access to the Internet. Early censors used simple
blocking techniques such as IP address blocking and DNS hijacking; hence, the
early circumvention tools are based on proxying the traffic to the blocked
destinations, i.e., by using an HTTP proxy \cite{RFC3143}. Examples of proxy-based
circumvention tools include Anonymizer~\cite{anonymizer}, Freenet~\cite{freenet}
and Ultrasurf~\cite{ultrasurf}, that helped a number of  users to
bypass the Internet censorship in the early days of Internet censorship.
Proxying network traffic is also adopted by the Tor anonymous communication
network \cite{dingledine:sec04} to help users bypass the censorship.
Tor bridges \cite{tor-bridge} proxy the censored clients'
traffic to the Tor network. The main challenge with the Tor bridges and other
proxy-based circumvention systems is that keeping the IP address of the proxies
unknown to the censors is a challenging problem
\cite{Sovran2008,McCoy2011,Feamster03,springerlink:10.1007/978-3-642-13122-6_29,McLachlan2009};
a censor learning the IP address of the proxies  can easily block any access to
them and also identify their users.

The use of more advanced technologies by the censors, e.g., content filtering using deep packet inspection, resulted in the emergence of more complicated circumvention systems \cite{infranet, collage, Karlin2011, Wustrow2011,Houmansadr2011a}. These systems aim in protecting their availability by hiding the use of their systems from the censors in the first place. As an example, Infranet~\cite{infranet} shares a secret key and some secret URL addresses with a client, which is then used to establish an unobservable communication between the client and the Infranet system, thereby enabling access the blocked destination. As another example, Collage~\cite{collage} works by having a client and the Collage system \textit{secretly} agree on some user-generated content sharing websites, e.g., flickr.com, and communicate using steganography. Unfortunately, sharing secret information with a wide range of clients is a serious challenge for these systems, as a censor can obtain the same secret information by pretending to be a client.

Some recent research suggests circumvention being built into the Internet infrastructure to better provide unobservability \cite{Karlin2011, Wustrow2011,Houmansadr2011a}. These systems rely on collaboration from some Internet routers that intercept users' traffic to uncensored destinations to establish covert communication between the users and the censored destinations. This provides a high degree of unobservability: a client's covert communication with a censored destination appears to the censor to be benign traffic with a non-prohibited destination. Telex~\cite{Wustrow2011} and Cirripede~\cite{Houmansadr2011a} provide this unobservable communication without the need for some pre-shared secret information with the client, as the secret keys are also covertly communicated inside the network traffic. Cirripede~\cite{Houmansadr2011a}  uses an additional client registration stage that provides some advantages and limitations as compared to Telex~\cite{Wustrow2011} and Decoy routing~\cite{Karlin2011} systems. Even though these systems are a large step forward in providing unobservable censorship circumvention their real-world deployment is highly dependent on collaboration from a number of ISPs/ASes, bringing into question whether they will be deployed in the near future.


\paragraphb{\name-like systems.} There are two projects that work in a similar manner to \name: the foe-project~\cite{foe} and the MailMyWeb~\cite{mailmyweb} for-profit service. Instead of tunneling traffic, which is the case in \name, these systems simply download a requested website and send it as an email attachment to the requesting user. This highly limits therir performance compared to \name, as discussed in Section~\ref{sec:mailmyweb}.



==> files/related_work.tex <==
\appendix


\section{Additional Related Work}
\label{sec:rltd}


%While we discuss the most closely related work in Section~\ref{sec:backgroundrw},
Here we provide some additional context on our work by overviewing the general area of covert communication.


%\subsection{Covert communication}
A covert channel provides the ability to hide the very existence of  messages by communicating them in a hidden manner through a legitimate channel, providing user unobservability. In this paper, we are interested in covert channels that use network flows as the communication medium. These covert channels can be broadly classified into two main classes: covert timing channels and covert storage channels. Timing channels send the covert message by making modifications to the arrival times of the network packets in a manner such that they are indistinguishable from the timings of benign packets \cite{cabuk:thesis06,Sellke2009}. As the existence of timing channels can be detected using different statistical tools \cite{Dartmouth:TR2005-536,CabBroShi04,GalatenkoGKT05,gian:ccs07} newer timing channels aim in matching a target timing distribution \cite{Gianvecchio2008,Liu:esorics09,Sellke2009}. Research \cite{conf/networking/ZanderAB11}  shows that such model-based timing channels may still be subject to detection due to imperfections in modeling network traffic.

Storage covert channels, on the other hand, exploit some packet fields that are either unused or pseudo-random \cite{Giffin2002,Murdoch2005,Zander:AB07}. As an example, the initial sequence number (ISN) field is a mandatory part of each TCP connection, and is generated in a pseudo-random manner by the TCP connection's end-hosts. This pseudo-random nature of the ISN provides an avenue to embed
covert traffic within the ISN \cite{Murdoch2005,Houmansadr2011a}. Other research suggests to use different fields of TCP/IP connections for covert communication, e.g., the IP's IPID~\cite{Murdoch2005}, TCP timestamps~\cite{Giffin2002}, and the TTL field of the IP header~\cite{Zander:AB07}.

The main limitation with the mentioned covert channels is their limited capacity for covert messages \cite{Sullivan98,Sellke2009}. As a result, such channels are not used in real-world scenarios for covert access to the Internet. As an example, the ISN-based covert channel of \cite{Murdoch2005} delivers only 24 bits of covert messages per each TCP connection. To overcome this limitation, recent research proposes to take advantage of the increasing use of encryption to build up high-capacity covert channels \cite{Wustrow2011,Karlin2011,Houmansadr2011a}.  More specifically, such research replaces the encrypted part of network traffic with the covert messages encrypted using a key not known to the adversary. For example, Telex~\cite{Wustrow2011},  Decoy Routing~\cite{Karlin2011} and Cirripede~\cite{Houmansadr2011a} replace the encrypted payload of HTTPS connections with covert messages, requiring assistance from cooperating ISPs to intercept these connections.
In our work, we use encrypted email communications as  a high capacity channel for the covert communication between users and our anti-censorship system, \name. By not requiring changes to the network architecture, \name can be easily deployed.


==> files/scheme.tex <==


\section{Threat model}\label{sec:model}

We assume that a user  is confined inside a censoring ISP, e.g., a user living under a repressive regime. The censoring ISP  blocks the user's access to certain Internet destinations, namely \textit{blocked destinations}. We assume that the censor uses today's advanced filtering technologies, including IP address blocking, DNS hijacking, and deep packet inspection techniques \cite{Leberknight2010}.  The censoring ISP also monitors all of its egress/ingress traffic to detect any use of circumvention techniques by  users that try to evade the censorship.

We assume that the censoring ISP's  censorship is constrained  not to
degrade the \textit{usability} of the Internet. In other words, even though
the censoring ISP \emph{selectively} blocks certain Internet connections, she is
not willing to block key Internet services \emph{entirely}. In particular, the operation
of \name system relies on the fact that a censoring ISP does not block \textit{all}
email communications, even though she can selectively block email messages/email providers.
We also assume that the censoring ISP  has as much information about \name as any \name client (\name does not share any secret information with its clients).

We also consider an active behavior for the censoring ISP.  An active censor, in addition to traffic monitoring,
%Moreover, our model includes an \textit{active adversarial} behavior for the censoring ISP: the censoring ISP
 manipulates its egress/ingress Internet traffic, e.g., by selectively dropping some packets, and adding additional latency to some packets,   in an attempt to disrupt the use of circumvention systems and/or to detect the users of such systems.
%This is in contrast to a \textit{passive censor} that only monitors the traffic.
Again, such perturbations are constrained to preserve the usability of the Internet for benign users.
%In other words, the censoring ISP does not manipulate the Internet traffic  in a way that  degrades the normal use of the Internet by its lawful users, due to various political and  business concerns.
%Many circumvention systems provide unobservability and/or availability to only a passive censor, whereas \name does so to both passive  and active censors.



\if 0
\section{Design goals}\label{sec:goals}


In this paper, we design and develop a censorship circumvention tool, called \name,
that uses open access to email services to provide an open access to the Internet.
In this section, we list and describe the key features that need to be considered in the design
and evaluation of an effective circumvention system. Later, in Section~\ref{sec:discussions}, we  evaluate these
features for the circumvention system designed in this paper.


%\begin{itemize}


\paragraph{Availability:}
Since censorship circumvention systems help users to evade Internet censorship, censoring ISPs
may try to block their users' access to such systems. As a result, an effective censorship circumvention
system should be difficult to block by censors.
Censors attempt to block the circumvention systems using techniques similar
to those used to censor the Internet, e.g., IP address blocking and deep packet inspection.
As we discuss later, we ensure the availability of our proposed system by binding it to the ability to use the Internet.


%One key mechanism to ensure availability for a circumvention system is to make
%communications with its users unobservable. As discussed above, many circumvention systems are not unobservable \cite{onion-routing,anonymizer}, and are hence prone to be easily blocked by censors.

\paragraph{Unobservability:} Usage unobservability is to disguise a user's
utilization of a circumvention system from the censorship authorities. The lack
of unobservability can result in identifying and, in some cases, penalizing the
users of circumvention systems.
Many existing circumvention
technologies do not provide high unobservability.
As an example, the widely used
HTTP proxies~\cite{RFC2616} easily give away the identities of their users once
they are detected by a censor; this is also true for  more complicated
proxy-based circumventions like Anonymizer~\cite{anonymizer} and the
Tor~\cite{onion-routing} network (we discuss this for the Tor bridges in Appendix~\ref{sec:rltd}).
Recent studies propose in-network circumventions that provide unobservability
to passive censorship, but not to the active censorship
\cite{Wustrow2011,Karlin2011,Houmansadr2011a}.

%\mattc{I removed some text here, as it sounded like it was arguing against
%the use of unobservability as an important goal. I think this paragraph
%should argue why unobservability is an important goal to have. I think the paragraph you had here %before in the begin\{comment\} does this better, why did you change it?}

% matt: I took out these two sentences. don't they argue against the use of your system? are they useful sentences to include here?
%In fact, as we discuss in Section~\ref{sec:enc}
%usage unobservability may only be a concern to specific citizens, e.g., political
%activists. To the best of our knowledge, there are no reports about normal
%citizen being arrested/penalized by repressive regimes as a result of using
%censorship circumvention systems.
%Many existing circumvention
%technologies do not provide high unobservability, yet they are regularly used
%by normal citizens under repressive regimes. As an example, the widely used
%HTTP proxies~\cite{RFC2616} easily give away the identities of their users once
%they are detected by a censor; this is also true for  more complicated
%proxy-based circumventions like Anonymizer~\cite{anonymizer} and the
%Tor~\cite{onion-routing} network (we discuss this for the Tor bridges later).
%Recent studies propose in-network circumventions that provide unobservability
%to passive censorship, but not to the active censorship
%\cite{Wustrow2011,Karlin2011,Houmansadr2011a}.

\begin{comment}
Users should be able to use a circumvention system in a way unobservable from their censoring ISPs.
The lack of unobservability can result in identifying, hence penalizing, the users of a circumvention system by a repressive regime that censors the Internet. Moreover, an observable circumvention system
generates communication patterns that can be used by a censoring ISP to block  access to it. As an example, some circumvention systems are accessible through  fixed, publicly known, sets of IP addresses \cite{onion-routing,anonymizer}, hence a censor can block their use by simply filtering their IP addresses.

A circumvention system's unobservability should be studied for both passive and active censors (as defined in Section~\ref{sec:model}).
Some systems provide unobservability to only passive censors~\cite{Wustrow2011,Karlin2011,Houmansadr2011a}.
\end{comment}

\paragraph{Ease of deployment:}
During the past decade, many designs have been proposed for circumvention systems,
while only a handful of them have been deployed and widely used in real-world.
There are several features that affect the deployment of a circumvention system. First,
some circumvention systems require modifications to the Internet infrastructure, which hinders their real-world deployment due to the lack of incentives from network operators and/or hardware/software vendors to apply these changes.
% Schemes that require changes to Internet routers or other network equipment hardware/software require cooperation from vendors, schemes that require configuration changes
%to networks require cooperation from operators of ISP networks, and schemes
%that require deployment within Internet services require cooperation
%from the Internet service provider.
%In other words, requiring support from third-party entities needs strong incentives matching the third party's business objectives, and
%there is often not enough incentives for these third parties to collaborate
%with circumvention systems.
As examples, several
recently-proposed schemes require help from web destinations \cite{infranet}
and ISPs \cite{Wustrow2011,Karlin2011,Houmansadr2011a} for their real-world deployment.
Second, a low-complexity design increases the chances that a system
will be deployed, as design
complexities can increase the effort and extent of changes required to deploy a system.
Finally, the amount of resources required by the system should be reasonable
(e.g., the number of physical machines required to support the system).


%the resources required by the system should be reasonable, e.g., the number of physical machines that
%run the system.
%Second, a design should be standalone, i.e., its deployment should not be bound to help and collaboration
%from other third-party entities, as usually there not enough incentives for the third-parties to collaborate with circumvention systems. As examples, several designs have been proposed that need help from some web destinations \cite{infranet} or some ISPs \cite{Wustrow2011,Karlin2011,Houmansadr2011a}.
%Third, a simple, working design increases the chances of the system to be deployed, as design
%complexities introduce different challenges regarding the real deployment of a circumvention system.



\paragraph{User convenience:}
A circumvention system should be easy to use for a wide range of users.
In other words, to receive high utilization by users, a circumvention system should require little technical knowledge and low resources  from its users. Ideally, a user should only need to install
the required circumvention software and configure it on her machine through a simple process, such that it can be used for a long period of time without the need for frequent manual reconfigurations and re-installations.



\paragraph{No reliance on shared secrets:}
Several circumvention systems share some secret information with their users~\cite{collage,infranet,tor-bridge}, e.g., secret design choices or secret keys, in order to provide service availability and/or unobservability. This introduces a new challenge to such systems as sharing secret information only with real users while keeping it secret from the censors is a hard problem, as discussed widely in the literature \cite{Sovran2008,McCoy2011,Feamster03,springerlink:10.1007/978-3-642-13122-6_29,McLachlan2009}.


\begin{comment}
To provide unobservability, several circumvention systems share some secret information with their intended users so that someone not having access to such information (e.g., a censor) will not be able to identify the users of such systems \cite{collage,infranet,tor-bridge}.
However, for such circumvention systems to be scalable there needs to be  mechanisms that ensures the exchange of
secret information only with the intended users, but not the censors; disclosure of the shared  secret information to the censors breaks the unobservability and availability promises of such circumvention systems. Sadly, this turns out to be a challenging open problem in the literature \cite{Sovran2008,McCoy2011,Feamster03,springerlink:10.1007/978-3-642-13122-6_29,McLachlan2009}.
\end{comment}


\begin{comment}
\paragraph{User anonymity:}
Even though the main incentive of using  censorship resistance systems is to acquire access to
censored regions of the Internet, many users prefer to anonymize their identity as well during their
use of circumvention systems. The reasons behind this is that some users do not fully trust the entity providing censorship resistance, some fear a security compromise in the circumvention   system, and some are not willing to reveal their identity to the final destination.
The use of anonymous communication systems like Tor \cite{onion-routing} and Anonymizer~\cite{anonymizer} for censorship circumvention provides user anonymity by itself,
however, many censorship resistance-specific systems \cite{infranet, collage,Wustrow2011,Houmansadr2011a} do not provide user anonymity (from the final destination or the circumvention system).
\end{comment}

%\end{itemize}

\fi






\section{Design of \name }\label{sec:scheme}
%the high level of our approach

In this section, we describe the detailed design of \name, our email-based censorship circumvention system.
Figure~\ref{fig:main} shows the overall architecture of \name. \name tunnels network connections between a client and a server, called \name server, inside email communications. The assumption that a censor does not block \emph{all} email communications, as stated in our threat model in Section~\ref{sec:model}, ensures a strong availability for \name since it does not rely on any specific email provider.
%As we assumed in the threat model before, all email traffic is not blocked by the censor and the use of encrypted email service  provides a plausible unobservability for  such a tunneled connection.
 Upon receiving the tunneled network packets, the \name server acts as a transparent proxy between the client and the network destinations requested by the client. In the following, we describe the detailed description of \name's client and server architectures.



%the service publices an email address, and runs server on multiple mail servers (can be made distrubuted)


% the client side
%(only need an email. no key or shared info
% needs to register at first with the email
% needs to


\subsection{\name server}\label{sec:server}



The \name server is a computer server running outside the censored region. The \name server helps a censored user to evade censorship
by proxying her traffic to blocked Internet destinations. More specifically, the \name server communicates with a  censored user by exchanging email messages that
carry network packets  of the user's tunneled traffic.
%\name server proxies the user's tunneled traffic to its final (blocked) destination.
Figure~\ref{fig:server} shows the building blocks of the \name server, which is composed of the following four main components:

\begin{figure}
\centering
 \includegraphics[width= \linewidth]{figs/server}
\caption{The main architecture  of \name server.}
\label{fig:server}
\end{figure}

 \noindent{\bf\ding{172} Email agent:} The email agent component  is an IMAP and SMTP server that receives email messages that  contain the tunneled Internet traffic, being sent by \name clients to \name's publicized email address {\tt tunnel@sweet.org}.
 The email agent passes the received email messages to another components of the \name server, i.e., the converter agent and the registration agent, to get processed accordingly.
The email agent also sends email messages to \name clients, which  are  generated by other components of \name server and contain tunneled network packets or client registration  information.
  %The email agent  also sends emails to \name client, containing the tunneled connections, which are generated by the converter component.

 \noindent{\bf \ding{173} Converter:} The converter component processes the emails passed by the email agent, and extracts the tunneled network packets. The converter, then, forwards the extracted data to another component of the \name server, the  proxy agent component.
 Also, the converter component receives network packets from the proxy agent and converts them into email messages
that are targeted to the email address of corresponding \name clients.
 The converter component then passes these email messages to the email agent for delivery to their intended recipients. As described later, the converter encrypts/decrypts the email attachments of a user using a secret key shared with that user.

 \noindent{\bf\ding{174} Proxy agent:} The proxy agent proxies the network packets of \name clients that are extracted by the converter component,
 and sends them to the Internet destination requested by the clients.
 In other words, the  proxy agent makes a proxy connection with \name clients, being tunneled inside the email-based communication.
 Through the established proxy connections, the client requests access to Internet destinations, e.g., blocked web sites.


\noindent{\bf\ding{175} Registration agent:} This component is in charge of registering the email addresses of the \name clients, prior to  their use of \name.
The information about the registered clients can be used to ensure quality of service for all users and prevent denial-of-service attacks on the
\name server. Additionally, the registration agent shares a secret key with the client, which is used to encrypt the tunneled information between the client and the \name server.



The email agent of the \name server receives two type of email messages; \textit{traffic emails}, which contain
tunneled traffic from the clients (sent to {\tt tunnel@sweet.org} address), and \textit{registration emails}, which carry client registration information (sent to {\tt register@sweet.org}).


\paragraphb{Client registration:} Before the very first use of the \name service,
a client needs to register her email address with the \name system. This is automatically
performed by the client's \name software, through the same email channel used for traffic tunneling. The objective of client registration is twofold: to prevent denial-of-service (DoS) attacks and to share a secret key between a client and the \name server.
A denial-of-service attack might  be launched on the \name server to disrupt its availability,
e.g., through sending many malformed emails on behalf of non-existing email addresses (this is discussed in Section~\ref{sec:discussions}). In order to register (or update) the email address of a client, the client's \name software sends a registration email from the user's email address, e.g., {\tt user@gmail.com}, to the \name's registration email
address, i.e., {\tt register@sweet.org}, requesting registration.
The email agent forwards all received registration emails to the registration agent (\ding{175})
of the \name server. For any new registration request, the registration agent generates and sends an email to the requesting email address (through the email agent) that contains a unique
computational \textit{challenge} (e.g., \cite{clientpuzzle}). After solving the challenge, the client software sends a second email  to
{\tt register@sweet.org} that contains the solution to the challenge, along with a Diffie-Hellman~\cite{dh} public key $K_C=g^{k_C}$.
If the client's response is verified by the registration agent the client's email address
will be added to a \textit{registration list}, that contains the list of registered email addresses with their expiration time. Also, the registration agent uses its own Diffie-Hellman public key, $K_R=g^{k_R}$, to evaluate a shared key $k_{C,R} = g^{k_R k_C}$ for the later communications with the client. The registration agent adds this key to the client's entry in the registration list, to be used for communications with that client. The client is able to generate the same $k_{C,R}$ key using \name's publicly advertised public key and her own private key \cite{dh}.

\paragraphb{Tunneling the traffic:} Any traffic email received by the email agent is processed as follows:
the email agent (\ding{172}) of \name server forwards the received traffic email to the converter agent (\ding{173}). The converter agent processes the traffic email and extracts the tunneled information from the email. The converter agent, then, decrypts the extracted traffic information (using the key $k_{C,R}$ corresponding to the user) and sends it to the  proxy agent (\ding{174}) of \name server. Finally, the  proxy processes the received packet as required, e.g., sends the packet to the requested destination.
Similarly, for any tunneled packet received from the proxied destinations, the proxy agent sends it to the converter agent. The converter agent encrypts the received packet(s) (using the corresponding $k_{C,R}$), and generate a traffic email that contain the encrypted data as email attachment. Each email is targeted to the email address of the corresponding client (e.g., by specifying the {\tt To:} field of the email message). The generated email is passed to the email agent, who sends the email to the corresponding client. Note that to improve the latency performance of the connection, small packets that arrive at the same time get attached to the same email message.



\subsection{\name client}\label{sec:client}

To use \name, a \name client needs to obtain a copy of  \name's client software and install it on her machine. The client further needs to have an email account with a public email provider, e.g.,  Gmail\footnote{\url{https://www.gmail.com}} mail service.
The choice of an encrypted versus plaintext email service makes a tradeoff between the usage unobservability and the performance. The use of an encrypted email service, e.g., Gmail, improves the usage unobservability while using a plaintext email service, e.g., Hotmail, improves the connection's throughput; this is discussed in Section~\ref{sec:enc}.
%To make the client's use of \name service unobservable to the censoring ISP, the client should use a public email account with encryption support.
%Also, the client's public email provider should reside outside the user's censoring ISP.
A client needs to configure the installed \name's software with information about her email account.
Prior to the first use of \name by a client, the client software registers the email address of its user with the \name server and obtains a shared secret key $k_{C,R}$, as described in Section~\ref{sec:server}.

We propose two designs for \name client software: a protocol-based design, which uses standard email protocols
to exchange email with client's email provider, and a webmail-based design, which uses the webmail interface of the client's email provider. We describe these two designs in the following.


\subsubsection{Protocol-based design}\label{sec:clientA}

Figure~\ref{fig:client1} shows the main elements of the protocol-based design of \name client. This is composed of three main components:

 \noindent{\bf\ding{182} Web Browser:} A \name client needs to use a web browser to render the web sites accessed through \name. The client can use any web browser that supports proxying of connections, e.g.,  Google Chrome, Internet Explorer, or Mozilla Firefox. The client needs to configure her web browser to use a local proxy server, e.g., by setting \code{localhost:4444} as the HTTP/SOCKS proxy in the browser's settings. The client can use two different web browsers for browsing with and without \name in order to avoid the need for frequent re-configurations of the browser. Alternatively, some browsers (e.g.,  Google Chrome , and Mozilla Firefox) allow a user to have multiple browsing \emph{profile}s, hence, a user can setup two profiles for browsing with and without \name.
% matt: I think some browswers (liek firefox) support Profiles -- could the user use the same browser but two profiles too?
%amir:great point! i added this

 \noindent{\bf\ding{183} Email Agent:} This component sends and receives \name emails thorough the client's public email account. The client needs to configure the email agent with the settings of the SMTP and IMAP/POP3 servers of her public email account. The client also needs to provide the email client with the required login information of her email account.

 \noindent{\bf\ding{184} Converter:} This component sits in the middle of the web browser and the email agent, and converts \name emails into network packets and vice versa. The converter uses the keys shared with \name, $k_{C,R}$, to encrypt/decrypt email contents.


Once the client enters a URL into the configured web browser (component \ding{182}), the browser makes a proxy connection to the local port that the converter (\ding{184}) is listening on (as specified in the proxy settings of the browser). The converter accepts the proxy connection from the browser and keeps the state of the established  TCP/IP connections. For packets that are received from the web browser the converter generates traffic emails, targeted to {\tt tunnel@sweet.org}, having the received packets as encrypted email attachments (using the key $k_{C,R}$). Such emails are passed to the email agent (\ding{183}) that sends the emails to the \name server through the public email provider of the client (as configured).

The email client is also configured to receive emails from the client's email account through an email retrieval protocol, e.g., IMAP or POP3. This allows the email agent to continuously look for new emails from the \name server. Once new emails are received the email agent passes them to the converter, who in turn extracts the packet information from the emails, decrypts them, and sends them to the web browser over the existing TCP/IP connection with the browser.





\begin{figure}
\centering
 \includegraphics[width= 1\linewidth]{figs/client1}
\caption{The protocol-based design for \name client.}
\label{fig:client1}
\end{figure}





\subsubsection{Webmail-based design}\label{sec:clientB}
As an alternative approach to the protocol-based design described above,  the \name client can use the webmail interface of the client's public email provider
to exchange emails with the \name server.

Figure~\ref{fig:client2} shows the main architecture of our webmail-based design. The main difference with the protocol-based design is that in this case the email agent (component \ding{183}) uses a web browser to exchange emails.
More specifically, the email agent uses its web browser to open a webmail interface with the client's email account, using the user's authentication credentials for logging in.
%To provide the required unobservability, the client should use an email account that provides HTTPS connectivity, e.g., Gmail's webmail.
Through this HTTP/HTTPS connection, the email agent communicates with the \name server by sending and receiving emails.
%The HTTPS connection with the public email provider hides client's communication with the \name system.
The rest of the webmail-based design is similar to the protocol-based design. If desired, the email agent can use the same web browser that the user uses for normal web browsing. %, i.e., not using \name.



\begin{figure}
\centering
 \includegraphics[width= 1\linewidth]{figs/client2}
\caption{The webmail-based design for \name client.}
\label{fig:client2}
\end{figure}

\subsection{The choice of the proxy protocol}
As mentioned before, the \name server uses a proxy agent that receives the tunneled traffic of
clients and establishes connections to the requested destinations. 
%In Section~\ref{sec:proxy} we mentioned different types of proxy servers that can be used to proxy Internet traffic. 
We consider the use of both SOCKS~\cite{RFC1928} and HTTP~\cite{RFC2616}  proxies in the design of \name, as each provides unique advantages. To provide the users with both options, our \name server's proxy agent runs a SOCKS proxy and an HTTP proxy in parallel, each running on a different port. A user can choose to use the type of proxy by configuring her \name client to connect to the corresponding port number.


The use of the SOCKS proxy  allows  the client to make \textit{any} IP connection through the \name system, including dynamic web communications, such as Javascript or AJAX, and instant messaging services. In contrast, an HTTP proxy only allows access to HTTP destinations. However, an HTTP proxy may speed up connections to such destinations by using HTTP-layer optimizations such as caching or pre-fetching of web objects.

%It should be noted that even though here we discuss web browsing through the \name client, the use of a SOCKS proxy allows the client to make any TCP/IP connection through the \name system, e.g., SSH connections. In Section ?? we investigate this for some applicaionts (???WE SHOULD DO THIS)
%\mattc{true, it would be cool to investigate this. If you don't have time, I think we should not use SSH as an example (4+ second lag times for SSH seem pretty unbearable, so I'm not convinced your scheme works for highly-interactive services like SSH. How about use "dynamic web communications, such as Javascript or AJAX" as an example? Or maybe instant messaging or IRC? More ideas: \url{http://en.wikipedia.org/wiki/List_of_TCP_and_UDP_port_numbers} }.

%\mattc{You should mention somewhere that your design is amenable to
%standard HTTP proxy tricks like web caching to reduce latency and bandwidth
%demands at the \name server.}

\subsection{An alternative approach: Web download}\label{sec:mailmyweb}

A trivial approach in providing censorship circumvention using email  is to download an entire webpage and attach it as an email attachment to email messages that are targeted to the requesting users. In fact, this approach is under development by the open-source foe project~\cite{foe}, and the  for-profit service of MailMyWeb~\cite{mailmyweb}.
%The main advantage of this approach over \name  is that fewer emails are required to be exchanged between the user and the anti-censorship system. 
Unfortunately, this simple approach only provides a limited access to the Internet: a user can only access static websites. In particular, this approach cannot be used to access destinations that require end-to-end encryption, contain dynamic web applications like HTML5 and Javascript sockets, or need user login information. Also, this approach does not support accessing web destinations that require a live Internet connection, e.g., video streaming websites, instant messaging, etc. In fact, the MailMyWeb service uses some heuristics to tackle some of these shortcomings partially, which are privacy-invasive and inefficient. For example, in order to access login-based websites MailMyWeb requests a user to send her login credentials to MailMyWeb by email. Also, a user can request for videos hosted \emph{only} on the YouTube video sharing website, which are then downloaded by MailMyWeb and sent as email attachments; this causes a large delay between the time a video is requested until it is has received by the user. \name, on the other hand, provides a comprehensive web browsing experience to its users since it can tunnel any kind of IP traffic.

%This web-download approach has been implemented as a commercial Internet service, called MailMyWeb\footnote{\url{http://www.mailmyweb.com/}}.
%MailMyWeb uses some tricks to tackle some of the mentioned limitations, e.g., it asks a  user willing to access a login-based website to email them her login credentials, which is not acceptable for many users.
%matt: I took out VoIP as an example. VoIP people argue that over 500ms (or is it 1s?) VoIP communication starts getting annoying, so I'm worried your current results (10 second RTTs) would make people think VoIP wouldn't work over your system




\if 0
\subsection{Alternative design choices}

In this paper, we proposed to tunnel Internet traffic inside email messages to evade censorship. To shed light on our design decisions,
we describe two alternative design decisions that could be incorporated
into \name. The first approach uses a different technique to tunnel traffic inside email communications. The second alternative uses
another type of Internet communication, with features similar to email communications, to tunnel Internet traffic.


%\mattc{This section argues why these alternative design choices aren't good ones to make. I think you don't need to do that. Instead, I think it would be better to argue that these alternative design choices have tradeoffs, and that the structure of your design is actually amenable to alternate forms of deployment if desired. I think it's actually a nice feature of your system if it's amenable to being deployed in different ways. If you do this, move MailMyWeb discussion elsewhere eg related work. } -- matt: let me think about this -- matt: meh, maybe the way you have it is fine actually. like nikita pointed out, one of your key benefits over MMW is dynamic communications like AJAX. So I think you should just skip my comment here (but I'll leave it here commented out in case it's useful for discussion later)


\subsubsection{Web download}\label{sec:mailmyweb}

A trivial approach in providing anti-censorship using email is to send the downloaded websites to the requesting users as an HTML, email attachment. More specifically, a user requesting access to a blocked destination, e.g., \url{http://blocked.com}, can send a single email to the email address publicized by the circumvention system. The circumvention system simply downloads \url{http://blocked.com} and sends a single email to the requesting user, including the downloaded website as an attachment. The main advantage of this approach over our \name approach is that fewer emails are required to be exchanged between the user and the anti-censorship system. However, this simple approach provides only limited access to the Internet: a user can only access static websites. More specifically, this approach cannot be used to access destinations that require end-to-end encryption, contain dynamic web applications like HTML5 or Javascript sockets, or need user login information. Also, this approach does not support accessing web destinations that require a live connection, e.g., video streaming websites, instant messaging, etc. %(MORE??)
This web-download approach has been implemented as a commercial Internet service, called MailMyWeb\footnote{\url{http://www.mailmyweb.com/}}.
MailMyWeb uses some tricks to tackle some of the mentioned limitations, e.g., it asks a  user willing to access a login-based website to email them her login credentials, which is not acceptable for many users.
%matt: I took out VoIP as an example. VoIP people argue that over 500ms (or is it 1s?) VoIP communication starts getting annoying, so I'm worried your current results (10 second RTTs) would make people think VoIP wouldn't work over your system





\subsubsection{Use of Instant Messaging  (IM) services }

Since Instant Messaging (IM) services exhibit lower transfer latencies as compared to emails, one could suggest to use IMs instead of emails in the design an anti-censorship system.
Several limitations and issues exist with the use of IMs for tunneling traffic that renders the use of it impractical for our anti-censorship application:

 \textbf{Rate limitation:} In order to avoid spamming activities, most IM providers limit the rate at which a client can send instant messages. As an example, IRC servers enforce a minimum delay of two seconds between any two consecutive IMs. Additionally, many IM providers temporarily suspend highly-active users for a specific time interval, e.g., the AOL Instant Messenger blocks a user for 30 seconds at a time once they have reached a maximum limit of messages. Such rate limitations make an IM-based circumvention system slower than our email-based system, \name.

\textbf{Lack of interoperability:} Unlike email, users on different instant messaging services are not usually able to communicate with each other, e.g., a user with a GTalk\footnote{\url{http://www.google.com/talk}} account can not directly send IMs to another user on  Yahoo! Messenger\footnote{\url{http://messenger.yahoo.com/}}. As a result, a \name-like system that uses IMs instead of email would require its users to only use IM services that are supported by its server. The public knowledge about the supported IM services can be used by a censor to block such an anti-censorship system by blocking the IM services supported by that service.
%This can also be used to identify the users of such anti-censorship systems.
This is in contrary to the use of emails, as used in our design, where a user can use \textit{any} email provider to get connected to \name.

 \textbf{Low data capacity:} The instant messaging services limit the amount of data being sent per each message. Such a limit ranges from 200 to 1000 characters, depending on the IM service provider. Combining this with the rate limitation, mentioned above, exhibits low data capacity for IM channels. This is in contrary to email communications that can carry attachments of tens of megabytes and are not limited in their rates, making it suitable for our purpose.


%\mattc{Do you know if IM services are encrypted? If not, maybe that's another downside (the censoring regime could see inside the instant messages)} Amir: some of them do support encryption  matt: oh, ok
\fi

